Exploring Scalability of Self-Training for Open-Vocabulary Temporal Action Localization

The vocabulary size in temporal action localization (TAL) is limited by the scarcity of large-scale annotated datasets. To overcome this, recent works integrate vision-language models (VLMs), such as CLIP, for open-vocabulary TAL (OV-TAL). However, despite the success of VLMs trained on extensive datasets, existing OV-TAL methods still rely on human-labeled TAL datasets of limited size to train action localizers, limiting their generalizability. In this paper, we explore the scalability of self-training with unlabeled YouTube videos for OV-TAL. Our approach consists of two stages: (1) a class-agnostic action localizer is trained on a human-labeled TAL dataset to generate pseudo-labels for unlabeled videos, and (2) the large-scale pseudo-labeled dataset is then used to train the localizer. Extensive experiments demonstrate that leveraging web-scale videos in self-training significantly enhances the generalizability of an action localizer. Additionally, we identify limitations in existing OV-TAL evaluation schemes and propose a new benchmark for thorough assessment. Finally, we showcase the TAL performance of the large multimodal model Gemini-1.5 on our new benchmark. Code is released at https://github.com/HYUNJS/STOV-TAL.

==> tab/recall_analysis.tex <==
\begin{wraptable}{r}[2mm]{4cm}
\vspace{-9mm}
% \hspace{-10mm}
\aboverulesep=0ex
\belowrulesep=0ex
% \setlength{\intextsep}{0pt}  % Space above and below the table
% \setlength{\columnsep}{20pt}  % Space between the text and the table
\setlength{\tabcolsep}{2pt} % Adjust the space between columns
\centering
\caption{
% Recall analysis on FineAction. R@1$\times$ is reported.
% Rec@1$\times$ on FineAction.
% Recall on FineAction.
\scriptsize Recall evaluation (FA).
}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c|}{tIoU@$0.5$} & \multicolumn{3}{c}{tIoU@Avg} \\
    & All & Base & Novel & All & Base & Novel \\
    \midrule
    ZS & 30.9 & 41.1 & 16.8 & 15.3 & 21.9 & 7.5 \\
    OV-ID & 30.5 & 40.8 & \textbf{17.0} & 15.2 & 21.6 & \textbf{8.1} \\
    OV-OD & \textbf{31.1} & \textbf{41.3} & 16.4 & \textbf{15.9} & \textbf{22.5} & 8.0 \\
    \bottomrule
\end{tabular}
}
\vspace{-8mm}
\label{tab:recall_analysis}
\end{wraptable}

% \begin{table}[t!]
% \vspace{-1mm}
% \aboverulesep=0ex
% \belowrulesep=0ex
% \setlength{\tabcolsep}{2pt} % Adjust the space between columns
% \centering
% \caption{
% Recall analysis on FineAction. R@1$\times$ is reported.
% }
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|ccc|ccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{3}{c|}{tIoU@$0.5$} & \multicolumn{3}{c}{tIoU@Avg} \\
%     & All & Base & Novel & All & Base & Novel \\
%     \midrule
%     ZS & 30.9 & 41.1 & 16.8 & 15.3 & 21.9 & 7.5 \\
%     OV-ID & 30.5 & 40.8 & \textbf{17.0} & 15.2 & 21.6 & \textbf{8.1} \\
%     OV-OD & \textbf{31.1} & \textbf{41.3} & 16.4 & \textbf{15.9} & \textbf{22.5} & 8.0 \\
%     \bottomrule
% \end{tabular}
% }
% \vspace{-6mm}
% \label{tab:recall_analysis}
% \end{table}

% \begin{table}[t!]
% \vspace{-1mm}
% \aboverulesep=0ex
% \belowrulesep=0ex
% \setlength{\tabcolsep}{2pt} % Adjust the space between columns
% \centering
% \caption{
% Recall analysis on FineAction. R@1$\times$ is reported.
% }
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|ccc|ccc}
%     \toprule
%     % \multirow{2}{*}{Method} & \multicolumn{3}{c|}{tIoU@$0.5$} & \multicolumn{3}{c}{tIoU@$[0.5:0.05:0.95]$} \\
%     \multirow{2}{*}{Method} & \multicolumn{3}{c|}{tIoU@$0.5$} & \multicolumn{3}{c}{tIoU@Avg} \\
%     & All & Base & Novel & All & Base & Novel \\
%     \midrule
%     % \baselineModel{} & 30.9 & 41.1 & 16.8 & 15.3 & 21.9 & 7.5 \\
%     % \ovidModel{} & 30.5 & 40.8 & \textbf{17.0} & 15.2 & 21.6 & \textbf{8.1} \\
%     % \ovodModel{} & \textbf{31.1} & \textbf{41.3} & 16.4 & \textbf{15.9} & \textbf{22.5} & 8.0 \\
%     ZS & 30.9 & 41.1 & 16.8 & 15.3 & 21.9 & 7.5 \\
%     OV-ID & 30.5 & 40.8 & \textbf{17.0} & 15.2 & 21.6 & \textbf{8.1} \\
%     OV-OD & \textbf{31.1} & \textbf{41.3} & 16.4 & \textbf{15.9} & \textbf{22.5} & 8.0 \\
%     \bottomrule
% \end{tabular}
% }
% \vspace{-6mm}
% \label{tab:recall_analysis}
% \end{table}
